BPS States in Omega Background and Integrability

We reconsider string and domain wall central charges in N=2 supersymmetric gauge theories in four dimensions in presence of the Omega background in the Nekrasov-Shatashvili (NS) limit. Existence of these charges entails presence of the corresponding topological defects in the theory - vortices and domain walls. In spirit of the 4d/2d duality we discuss the worldsheet low energy effective theory living on the BPS vortex in N=2 Supersymmetric Quantum Chromodynamics (SQCD). We discuss some aspects of the brane realization of the dualities between various quantum integrable models. A chain of such dualities enables us to check the AGT correspondence in the NS limit.

==> cover.tex <==
Title:
BPS States in Omega Background and Integrability

Authors:
Kseniya Bulycheva, Heng-yu Chen, Alexander Gorsky, and Peter Koroteev

Report numbers:
UMN-TH-3108/12, FTPI-MINN-12/21, NSF-KITP-12-108, ITEP-TH-30/12

47 pages 10 figures

Abstract:
We reconsider string and domain wall central charges in $\mathcal{N}=2$ supersymmetric gauge theories in four dimensions in presence of the Omega background in the Nekrasov-Shatashvili (NS) limit. Existence of these charges entails presence of the corresponding topological defects in the theory -- vortices and domain walls. In spirit of the 4d/2d duality we discuss the worldsheet  low energy effective theory living on the BPS vortex in $\mathcal{N}=2$ Supersymmetric Quantum Chromodynamics (SQCD). We discuss some aspects of the brane realization of the dualities between various quantum integrable models. A chain of such dualities enables us to check the AGT correspondence in the NS limit.
